Higher-Group Statistics on Lattices

Crossing a domain wall can permute anyons, and intersecting strings can create a particle. These couplings between defects of various dimensions are specified by higher groups. We develop a lattice framework defining higher-group statistics as Berry phases of closed sequences of hopping operators, invariant under local modifications of the operators. Our central example is a closed Majorana chain, a 1-dimensional topological superconductor, embedded in 3 dimensions. We construct a loop-flip process with phase $+i$, refining the usual $\pm 1$ loop-flip invariant through intermediate transfer of fermion parity between the chain and physical fermions. In two dimensions, charge-wall statistics distinguish two $\mathbb Z_4$ toric codes enriched by $\mathbb Z_2$ charge-conjugation symmetry, with identical anyon statistics but distinct gauged theories: the quantum doubles of the dihedral group $D_4$ and the quaternion group $Q_8$. We provide two complementary constructions of statistical processes. The first extends the Smith normal form algorithm in [Phys. Rev. X $\textbf{16}$, 011010 (2026), arXiv:2412.01886] to higher groups, generating processes from lattice geometry and prescribed local moves. For a finite higher group $\mathbb G$, we prove that statistical processes on a $d$-sphere are classified by $H_{d+2}(B\mathbb G,\mathbb Z)$. The second constructs processes directly from homology classes without examining exponentially many defect configurations, enabling us to study statistics for complex higher-group structures where the previous method is computationally prohibitive. These processes detect boundary anomalies of higher-group symmetry-protected topological phases. For example, we distinguish 2-group anomalies in 1, 2, and 3 dimensions. Higher-group statistics provide new invariants for characterizing coupled defects in quantum many-body systems.

==> figures/inversion_dual_geometry.tex <==
\providecommand{\invDualCoordinates}{%
 \coordinate (p0) at (-2.65,-.85);
 \coordinate (p1) at ({2*sqrt(3)/5},.4);
 \coordinate (p2) at ({-2*sqrt(3)/5},.4);
 \coordinate (p3) at (0,-.8);
 \coordinate (q0) at (0,0);
 \coordinate (q1) at ({-sqrt(3)*43/40},-1.075);
 \coordinate (q2) at ({sqrt(3)*43/40},-1.075);
 \coordinate (q3) at (0,2.15);
}%
\providecommand{\invDualBlackPaths}[1]{%
 \draw[#1] (p1)--(p2)--(p3)--cycle;
}%
\providecommand{\invDualBlackCompletionPaths}[1]{%
 \draw[#1] (p3) .. controls (-.65,-1.85) and (-1.85,-1.65) .. (p0);
 \draw[#1] (p2) .. controls (-1.45,.80) and (-2.55,.20) .. (p0);
 \draw[#1] (p1) .. controls (2.20,.80) and (1.35,2.75) .. (0,2.75)
   .. controls (-2.65,2.75) and (-3.20,.55) .. (p0);
}%
\providecommand{\invDualFullBlackPaths}[1]{%
 \invDualBlackPaths{#1}
 \invDualBlackCompletionPaths{#1}
}%
\providecommand{\invDualBluePaths}[1]{%
 \foreach \a/\b in {0/1,0/2,0/3,1/2,1/3,2/3}{%
  \draw[#1] (q\a)--(q\b);
 }
}%
\providecommand{\invDualBoundary}[1]{%
 \draw[#1] (p1)--(p2)--(p3)--cycle;
}%
\endinput

